Dynamic Diffuse Global Illumination Resampling

Interactive global illumination remains a challenge in radiometrically- and geometrically-complex scenes. Specialized sampling strategies are effective for specular and near-specular transport because the scattering has relatively low directional variance per scattering event. In contrast, the high variance from transport paths comprising multiple rough glossy or diffuse scattering events remains notoriously difficult to resolve with a small number of samples. We extend unidirectional path tracing to address this by combining screen-space reservoir resampling and sparse world-space probes, significantly improving sample efficiency for transport contributions that terminate on diffuse scattering events. Our experiments demonstrate a clear improvement -- at equal time and equal quality -- over purely path traced and purely probe-based baselines. Moreover, when combined with commodity denoisers, we are able to interactively render global illumination in complex scenes.

==> fig_denoised.tex <==
%!TEX root = paper.tex
% DO NOT EDIT---This file is generated using scripts\fig_denoised.py
\setlength{\fboxrule}{1pt}%
\setlength{\tabcolsep}{1pt}%
\renewcommand{\arraystretch}{1}%
\small%
\centering%
\begin{tabular}{cccccccc}%
            DDGI
                    &
                    Indirect (Ours)
                    &
                    +Resampling
                    & Reference
                \\%
    \multicolumn{4}{c}{\setlength{\fboxsep}{1.5pt}\begin{overpic}[width=\linewidth]{figures/fig_denoised/combined_greek_villa.jpg}
        %\put(8, 43) { \colorbox{black}{\textcolor{white}{Path tracing}} }
        %\put(11.5, 40) { \colorbox{black}{\textcolor{white}{0.0673 / 24.6 ms}} }
        %\put(44, 43) { \colorbox{black}{\textcolor{white}{+ ReSTIR}}  }
        %\put(46, 40) { \colorbox{black}{\textcolor{white}{0.0517 / 25.6 ms}}  }
        %\put(74, 43) { \colorbox{black}{\textcolor{white}{+ NRC (Ours)}} }
        %\put(79, 40) { \colorbox{black}{\textcolor{white}{0.0521 / 38.4 ms}} }
        \put(28.59375, 22.083333333333336){\makebox(0,0){\tikz\draw[red,ultra thick] (0,0) rectangle (0.10312500000000001\linewidth, 0.041249999999999995\linewidth);}}
        \put(62.34375, 8.333333333333337){\makebox(0,0){\tikz\draw[orange,ultra thick] (0,0) rectangle (0.10312500000000001\linewidth, 0.041249999999999995\linewidth);}}
        \put(73.69791666666666, 28.749999999999996){\makebox(0,0){\tikz\draw[yellow,ultra thick] (0,0) rectangle (0.10312500000000001\linewidth, 0.041249999999999995\linewidth);}}
    \end{overpic}}
    \\%
    \fcolorbox{red}{red}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_0_0.jpg}} &
    \fcolorbox{red}{red}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_1_0.jpg}} &
    \fcolorbox{red}{red}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_2_0.jpg}} &
    \fcolorbox{red}{red}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_3_0.jpg}}
    \\%
    \fcolorbox{orange}{orange}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_0_1.jpg}} &
    \fcolorbox{orange}{orange}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_1_1.jpg}} &
    \fcolorbox{orange}{orange}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_2_1.jpg}} &
    \fcolorbox{orange}{orange}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_3_1.jpg}}
    \\%
    \fcolorbox{yellow}{yellow}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_0_2.jpg}} &
    \fcolorbox{yellow}{yellow}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_1_2.jpg}} &
    \fcolorbox{yellow}{yellow}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_2_2.jpg}} &
    \fcolorbox{yellow}{yellow}{\includegraphics[width=0.236\linewidth]{figures/fig_denoised/inset_greek_villa_3_2.jpg}}
    \\%
            DDGI
                    &
                    Indirect (Ours)
                    &
                    +Resampling
                    & Reference
                \\%
            0.0673 / 24.6 ms&
            0.0517 / 25.6 ms&
            0.0521 / 38.4 ms&
        \\%
\end{tabular}

==> fig_main_result.tex <==
%!TEX root = paper.tex
% DO NOT EDIT---This file is generated using .\scripts\fig_main_result.py
\setlength{\fboxrule}{10pt}%
\setlength{\insetvsep}{20pt}%
\setlength{\tabcolsep}{-0.1pt}%
\renewcommand{\arraystretch}{1}%
\footnotesize%
\hspace*{0.5mm}\begin{tabular}{lcccccc}
    &Reference
    &Path tracing
    &Direct DDGI
    &Indirect DDGI
    &+Resampling (Ours)
    &Reference
    \\%
    \setInset{A}{red}{520}{450}{244}{120}%
    \setInset{B}{orange}{1100}{800}{326}{160}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-17mm}\ZeroDay}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/measure_seven/ref.jpg}{0.263}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/measure_seven/direct.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/measure_seven/indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/measure_seven/ourc-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/measure_seven/ours-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/measure_seven/ref.jpg}%
    \\%
    & MRSE / Framerate:
    &0.09 / 28.7 fps%
    &0.20 / 60.1 fps%
    &0.24 / 47.9 fps%
    &0.24 / 36.4 fps%
    &%
    \\%
    \setInset{A}{red}{100}{270}{244}{120}%
    \setInset{B}{orange}{1150}{750}{326}{160}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-18mm}\LivingRoom}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/living_room/ref.jpg}{0.263}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/direct.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/ourc-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/ours-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/ref.jpg}%
    \\%
    & MRSE / Framerate:
    &0.31 / 62.5 fps%
    &0.03 / 98.0 fps%
    &1.57 / 66.0 fps%
    &0.13 / 43.8 fps%
    &%
    \\%
    \setInset{A}{red}{310}{480}{244}{120}%
    \setInset{B}{orange}{1100}{650}{489}{240}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-14mm}\PinkRoom}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/pink_room/ref.jpg}{0.263}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/direct.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/ourc-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/ours-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/ref.jpg}%
    \\%
    & MRSE / Framerate:
    &0.08 / 69.9 fps%
    &0.26 / 91.8 fps%
    &0.28 / 69.7 fps%
    &0.29 / 39.9 fps%
    &%
    \\%
    \setInset{A}{red}{900}{400}{244}{120}%
    \setInset{B}{orange}{1050}{750}{326}{160}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-18mm}\RoomDoor}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/room_door/ref.jpg}{0.263}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/direct.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/ourc-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/ours-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/ref.jpg}%
    \\%
    & MRSE / Framerate:
    &0.66 / 237 fps%
    &0.04 / 122 fps%
    &0.05 / 91.6 fps%
    &0.02 / 43.7 fps%
    &%
    \\%
    \setInset{A}{red}{350}{780}{326}{160}%
    \setInset{B}{orange}{750}{800}{326}{160}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-18mm}\SplitRoom}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/occlusion_resampling/ref.jpg}{0.263}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/direct.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/ourc-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/ours-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/ref.jpg}%
    \\%
    & MRSE / Framerate:
    &0.09 / 228 fps%
    &0.22 / 141 fps%
    &0.03 / 90.6 fps%
    &0.02 / 54.9 fps%
    &%
    \\%
    \setInset{A}{red}{700}{500}{326}{160}%
    \setInset{B}{orange}{1250}{600}{326}{160}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-18mm}\RedBall}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/simple_resampling/ref.jpg}{0.263}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/direct.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/ourc-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/ours-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/ref.jpg}%
    \\%
    & MRSE / Framerate:
    &0.03 / 274 fps%
    &0.02 / 145 fps%
    &0.03 / 94.4 fps%
    &0.03 / 58.5 fps%
    &%
    \\%
\end{tabular}

==> fig_main_result_128.tex <==
%!TEX root = paper.tex
% DO NOT EDIT---This file is generated using scripts\fig_main_result.py
\setlength{\fboxrule}{10pt}%
\setlength{\insetvsep}{20pt}%
\setlength{\tabcolsep}{-0.1pt}%
\renewcommand{\arraystretch}{1}%
\footnotesize%
\hspace*{0.5mm}\begin{tabular}{lccccccc}
    &Reference
    &DDGI
    &PT
    &Indirect DDGI
    &+Resampling (Ours)
    &+Bounding (Ours)
    &Reference
    \\%
    \setInset{A}{red}{679}{635}{244}{120}%
    \setInset{B}{orange}{1190}{625}{326}{160}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-17mm}\PinkRoom}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/pink_room/ref.jpg}{0.23}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/ddgi.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/pt.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/ddgi-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/ddgi-indirect-resampled.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/ddgi-indirect-resampled-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/pink_room/ref.jpg}%
    \\%
    & MAPE / Frametime (ms):
    &0.33 / 19.0 ms%
    &0.03 / 108 ms%
    &0.18 / 21.4 ms%
    &0.14 / 29.9 ms%
    &0.14 / 31.1 ms%
    &%
    \\%
    \setInset{A}{red}{100}{270}{244}{120}%
    \setInset{B}{orange}{544}{694}{326}{160}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-18mm}\LivingRoom}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/living_room/ref.jpg}{0.23}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/ddgi.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/pt.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/ddgi-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/ddgi-indirect-resampled.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/ddgi-indirect-resampled-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/living_room/ref.jpg}%
    \\%
    & MAPE / Frametime (ms):
    &0.32 / 21.7 ms%
    &0.17 / 122 ms%
    &0.32 / 24.2 ms%
    &0.38 / 33.4 ms%
    &0.38 / 32.8 ms%
    &%
    \\%
    \setInset{A}{red}{425}{362}{244}{120}%
    \setInset{B}{orange}{1025}{530}{489}{240}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-14mm}\GreekVilla}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/greek_villa/ref.jpg}{0.23}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/greek_villa/ddgi.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/greek_villa/pt.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/greek_villa/ddgi-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/greek_villa/ddgi-indirect-resampled.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/greek_villa/ddgi-indirect-resampled-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/greek_villa/ref.jpg}%
    \\%
    & MAPE / Frametime (ms):
    &0.50 / 20.0 ms%
    &0.19 / 106 ms%
    &0.39 / 23.6 ms%
    &0.37 / 29.7 ms%
    &0.37 / 29.4 ms%
    &%
    \\%
    \setInset{A}{red}{1032}{382}{244}{120}%
    \setInset{B}{orange}{389}{177}{326}{160}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-18mm}\RoomDoor}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/room_door/ref.jpg}{0.23}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/ddgi.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/pt.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/ddgi-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/ddgi-indirect-resampled.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/ddgi-indirect-resampled-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/room_door/ref.jpg}%
    \\%
    & MAPE / Frametime (ms):
    &3.76 / 16.2 ms%
    &0.09 / 50.5 ms%
    &3.64 / 17.9 ms%
    &3.65 / 27.4 ms%
    &3.66 / 28.8 ms%
    &%
    \\%
    \setInset{A}{red}{350}{780}{326}{160}%
    \setInset{B}{orange}{750}{800}{326}{160}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-18mm}\SplitRoom}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/occlusion_resampling/ref.jpg}{0.23}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/ddgi.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/pt.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/ddgi-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/ddgi-indirect-resampled.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/ddgi-indirect-resampled-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/occlusion_resampling/ref.jpg}%
    \\%
    & MAPE / Frametime (ms):
    &0.25 / 15.1 ms%
    &0.04 / 24.5 ms%
    &1.02 / 16.4 ms%
    &0.06 / 22.4 ms%
    &0.06 / 23.4 ms%
    &%
    \\%
    \setInset{A}{red}{928}{90}{326}{160}%
    \setInset{B}{orange}{1286}{713}{326}{160}%
    \hspace{-4mm}\rotatebox{90}{\hspace{-18mm}\RedBall}%
    &\addBeautyCrop{generated_figures/fig_main_result_128/simple_resampling/ref.jpg}{0.23}{1920}{1080}{0}{0}{1920}{1080}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/ddgi.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/pt.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/ddgi-indirect.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/ddgi-indirect-resampled.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/ddgi-indirect-resampled-bounded.jpg}%
    &\addInsets{generated_figures/fig_main_result_128/simple_resampling/ref.jpg}%
    \\%
    & MAPE / Frametime (ms):
    &0.19 / 15.9 ms%
    &0.02 / 24.8 ms%
    &0.85 / 17.4 ms%
    &0.03 / 25.5 ms%
    &0.03 / 26.4 ms%
    &%
    \\%
\end{tabular}
